A 3/2-approximation algorithm for the Student-Project Allocation problem

The Student-Project Allocation problem with lecturer preferences over Students (SPA-S) comprises three sets of agents, namely students, projects and lecturers, where students have preferences over projects and lecturers have preferences over students. In this scenario we seek a stable matching, that is, an assignment of students to projects such that there is no student and lecturer who have an incentive to deviate from their assignee/s. We study SPA-ST, the extension of SPA-S in which the preference lists of students and lecturers need not be strictly ordered, and may contain ties. In this scenario, stable matchings may be of different sizes, and it is known that MAX SPA-ST, the problem of finding a maximum stable matching in SPA-ST, is NP-hard. We present a linear-time 3/2-approximation algorithm for MAX SPA-ST and an Integer Programming (IP) model to solve MAX SPA-ST optimally. We compare the approximation algorithm with the IP model experimentally using randomly-generated data. We find that the performance of the approximation algorithm easily surpassed the 3/2 bound, constructing a stable matching within 92% of optimal in all cases, with the percentage being far higher for many instances.

==> spare.tex <==
describes a $3/2$-approximation algorithm for finding a maximum stable matching for instances of the \emph{Stable Marriage problem with Ties and Incomplete lists} (\acrshort{smti}). \acrshort{smti} may be seen as a special case of \acrshort{spa-st} in which lecturers do not exist and projects have preferences over students with no agent having an upper quota greater than $1$. Kir\'{a}ly \cite{ZK} also provided a $3/2$-approximation algorithm to find a maximum stable matching for instances of the \emph{Hospitals/Residents problem with ties} (\acrshort{hrt}), where \acrshort{hrt} is an extension of \acrshort{smti} in which upper quotas greater than $1$ are allowed for one type of agent. \acrshort{hrt} is also a special case of \acrshort{spa-st}. An \acrshort{hr} instance is identical to an \acrshort{hrt} instance except ties are not allowed in preference lists. For both \acrshort{hr} \cite{DG_LS} and \acrshort{spa-s} \cite{DA_KC_DM_KM} instances, a stable matching can always be found in linear time with the property that for each instance all stable matchings are the same size.

\subsection{Related work}

%\acrshort{spa-p} is a similar problem to \acrshort{spa-st} in which there are no ties in preference lists and lecturers have preferences over projects rather than students. In \acrshort{spa-p} stable matchings may be of different sizes and the problem of finding a maximum sized stable matching is also NP-hard \cite{DM_GOM}. Manlove and O'Malley \cite{DM_GOM} showed that any stable matching in \acrshort{spa-p} is a 2-approximation to the maximum stable matching. It is straightforward to draw a corresponding proof for instances of \acrshort{spa-st} from this.
 
Kir\'{a}ly \cite{ZK} describes a $3/2$-approximation algorithm for finding a maximum stable matching for instances of the \emph{Stable Marriage problem with Ties and Incomplete lists} (\acrshort{smti}). \acrshort{smti} may be seen as a special case of \acrshort{spa-st} in which lecturers do not exist and projects have preferences over students with no agent having an upper quota greater than $1$. Kir\'{a}ly \cite{ZK} also provided a $3/2$-approximation algorithm to find a maximum stable matching for instances of the \emph{Hospitals/Residents problem with ties} (\acrshort{hrt}), where \acrshort{hrt} is an extension of \acrshort{smti} in which upper quotas greater than $1$ are allowed for one type of agent. \acrshort{hrt} is also a special case of \acrshort{spa-st}. An \acrshort{hr} instance is identical to an \acrshort{hrt} instance except ties are not allowed in preference lists. For both \acrshort{hr} \cite{DG_LS} and \acrshort{spa-s} \cite{DA_KC_DM_KM} instances, a stable matching can always be found in linear time with the property that for each instance all stable matchings are the same size.

It was necessary to check whether there was a simple way to transform an instance $I$ of \acrshort{spa-st} into an instance $I'$ of \acrshort{smti}, use the existing algorithm and then covert the resulting stable matching back. In order to test this a natural cloning technique to convert instances of \acrshort{spa-st} into instances of \acrshort{hrt} was created and is described in Appendix \ref{cloning_spast_smti}. An existing technique was then used to further convert these \acrshort{hrt} instances to an \acrshort{smti} instances. It was found that not only does a stable matching in $I'$ does not necessarily equate to a stable matching in $I$, but also in cases where this conversion does hold, the $\frac{3}{2}$ bound is not assured. This motivates the need for a bespoke algorithm for the more general \acrshort{spa-st} case.

